Breaking The Dimension Dependence in Sparse Distribution Estimation under Communication Constraints

We consider the problem of estimating a $d$-dimensional $s$-sparse discrete distribution from its samples observed under a $b$-bit communication constraint. The best-known previous result on $\ell_2$ estimation error for this problem is $O\left( \frac{s\log\left( {d}/{s}\right)}{n2^b}\right)$. Surprisingly, we show that when sample size $n$ exceeds a minimum threshold $n^*(s, d, b)$, we can achieve an $\ell_2$ estimation error of $O\left( \frac{s}{n2^b}\right)$. This implies that when $n>n^*(s, d, b)$ the convergence rate does not depend on the ambient dimension $d$ and is the same as knowing the support of the distribution beforehand. We next ask the question: ``what is the minimum $n^*(s, d, b)$ that allows dimension-free convergence?''. To upper bound $n^*(s, d, b)$, we develop novel localization schemes to accurately and efficiently localize the unknown support. For the non-interactive setting, we show that $n^*(s, d, b) = O\left( \min \left( {d^2\log^2 d}/{2^b}, {s^4\log^2 d}/{2^b}\right) \right)$. Moreover, we connect the problem with non-adaptive group testing and obtain a polynomial-time estimation scheme when $n = \tilde{\Omega}\left({s^4\log^4 d}/{2^b}\right)$. This group testing based scheme is adaptive to the sparsity parameter $s$, and hence can be applied without knowing it. For the interactive setting, we propose a novel tree-based estimation scheme and show that the minimum sample-size needed to achieve dimension-free convergence can be further reduced to $n^*(s, d, b) = \tilde{O}\left( {s^2\log^2 d}/{2^b} \right)$.

==> sec_introduction.tex <==
Distributed estimation is a central task in modern data science, where datasets are often either generated from distributed sources such as smartphones and wireless sensors, or are too large to be stored on a centralized machine. When data is distributed across multiple devices, communication cost often becomes a bottleneck of modern machine learning tasks \citep{Feng11}. This is even more so in federated analytic type settings, where communication occurs over bandwidth-limited wireless links such as in federated learning \citep{kairouz2019advances}. For several statistical inference tasks, including distribution estimation, communication constraint is shown to result in drastic performance drop (see Section~\ref{sec:related_works} for more details) if we do not have any further assumption on the data distribution. However, in many real-world applications, the underlying distribution is often supported only on a sparse but unknown subset of the domain. By leveraging the sparse structure of data, we can significantly improve the performance of estimating discrete distribution \citep{acharya2020estimating}.

Without the sparse assumption, the $\ell_2$ estimation error can be as large as $O\lp \frac{d}{n2^b}\rp$ \citep{han2018distributed}, which is undesired as in many applications $d$ can be much larger than the sample size $n$. With the $s$-sparse assumption, on the other hand, one can view $p \in \mcal{P}_{s, d}$ as a sparse vector and apply any compressed sensing (CS) based method \citep{donoho2006compressed, candes2006stable} to losslessly compress the vector into a $s\log d$-dimensional vector. Therefore a natural  approach is as follows: let $M$ be a CS measurement matrix, and each client first compresses their local observation $X_i$ to $M\cdot X_i \in \mbb{R}^{c_0s\log\lp d/s \rp \times 1}$ (where we treat $X_i$ as a $d$-dim one-hot vector). Under a $1$ bit communication constraint, client $i$ randomly samples $1$ (out of $c_0s\log (d/s)$) coordinate from $M\cdot X_i$, quantizes it to $1$ bit, and then sends it to the server. Under this subsampled-and-quantized approach (\citep{chen2020breaking}), the equivalent sample size (i.e. the number of participating clients) is discounted by a factor of $s\log\lp {d}/{s} \rp$ (due to the subsampling step), resulting in $\ell_2$ error $O\lp\frac{s\log(d/s)}{n} \rp$. Indeed, this approach is used in sparse distribution estimation under privacy constraint \citep{xiong2020compressive}. Even when one uses random hash functions (such as count-sketch based approach in \citep{Bassily2017}) and does a more careful analysis, we still end up with a dependency of $O\lp \frac{s\log\lp d/s\rp}{n2^b}\rp$-- see \citep{acharya2020estimating} for more details. Therefore, the logarithmic dependency on $d$ seems natural and inevitable.

In this work, however, we surprisingly prove that one can eliminate the $\log\lp {d}/{s} \rp$ term and achieve a \emph{dimension-free}\footnote{This means that the convergence rate does not depend on the ambient dimension $d$.} convergence rate $O\lp \frac{s}{n2^b} \rp$, as long as $n$ is larger than a threshold $n^*(s, d, b)$. This closes the multiplicative $\log\lp {d}/{s}\rp$ gap between the upper and lower bounds in \citep{acharya2020estimating}. To achieve $O\lp \frac{s}{n2^b} \rp$ convergence, we propose a two-stage scheme that consists of a concatenation of two generic sub-schemes. For the first stage, use the first $n_1$ samples (clients) to \emph{localize} the support of $p$ (denoted as $\msf{supp}(p)$), and then use the second $n-n_1$ samples to refine the estimation. By carefully designing the localization stage, we improve the best-known result $O\lp\frac{s\log(d/s)}{n2^b} \rp$ to $O\lp \frac{s}{n2^b}\rp$.  Notice that $O\lp \frac{s}{n2^b}\rp$ is optimal since it is also the minimax convergence rate when $\msf{supp}(p)$ is given beforehand \citep{han2018distributed, barnes2019lower, han2018geometric}, and to our best knowledge, this is the first work that observes such dimension independent convergence. Therefore, for the sparse distribution estimation task, instead of investigating the optimal convergence rate, the correct question to ask is \emph{``what is the minimum sample size $n^*(s,d,b)$ required in order to achieve the dimension-free convergence rate $O\lp \frac{s}{n2^b}\rp$?''} 

%To achieve $\Omega\lp \frac{s}{n2^b} \rp$ convergence, we propose a two-stage scheme that consists of a concatenation of two generic sub-schemes. For the first stage, use the first $n_1$ samples (clients) to \emph{localize} the support of $p$ (denoted as $\msf{supp}(p)$), and then use the second $n-n_1$ samples to refine the estimation. By carefully designing the localization sub-scheme, we improve the best known result $O\lp\frac{s\log(d/s)}{n2^b} \rp$ to $O\lp \frac{s}{n2^b}\rp$, closing the gap in \citep{acharya2020estimating}. To our best knowledge, this is the first work that observes such dimensional independent convergence. Notice that $O\lp \frac{s}{n2^b}\rp$ is optimal since it is also the minimax convergence rate when $\msf{supp}(p)$ is given beforehand \citep{han2018distributed, barnes2019lower, han2018geometric}. Therefore, for the sparse distribution estimation task, instead of investigating the optimal convergence rate, the correct question to ask is \emph{"what is the minimum sample size $n^*(s,d,b)$ required in order to achieve the dimension-free convergence rate $O\lp \frac{s}{n2^b}\rp$?"} 

For non-interactive setting (where each client encodes her observation independently), a careful extension of the grouping approach studied in \citep{han2018distributed} leads to an upper bound of $n^*(s, d, b) = O\lp {d^2\log^2 d}/{2^b} \rp$. On the other hand, by using a clever construction of random hash functions in the localization step, we show that $n^*(s, d, b) = O\lp {s^4\log^2 d}/{2^b} \rp$, which depends only logarithmically on $d$. Nevertheless, the decoding algorithm involves searching all possible $s$-sparse supports and is computational inefficient. To resolve the computational issue, we make a non-trivial connection to non-adaptive group testing, showing that as long as $n = \tilde{\Omega}\lp {s^4\log^4 d}/{2^b}\rp$\footnote{For ease of presentation, we use the notation $\tilde{O}(\cdot)$ and $\tilde{\Omega}(\cdot)$ to hide all dependence on $\log s$ and $\log\log d$.}, we can achieve the optimal estimation error in polynomial time. %Finally, we give a lower bound on $n^*(s, d,b)$ for non-interactive schemes, showing that $n^*(s, d,b)$ is at least $\tilde{\Omega}\lp s^2 \rp$. 
For sequentially interactive scheme, we propose a tree-based scheme that achieves optimal convergence rate when $n = \tilde{\Omega}\lp{ s^2\log^2 d}/{2^b}\rp$, showing that interactivity can benefit the minimum required sample size.

Several extensions are also studied. First, when the data is \emph{distribution-free} and the goal is to estimate the empirical frequency of symbols, our schemes extend naturally and all the convergence guarantees hold as in the distributional settings. Second, when $p$ is \emph{almost-sparse}, our schemes work as well, and we give an upper bound on the estimation error.  Finally, by using state-of-the-art non-adaptive group testing results, one can reduce the decoding complexity to $\msf{poly}(s, \log d)$ for the $1$-bit case. Extending to $b$-bit, however, remains unsettled and is left as a future work.

To summarize, our main technical contributions include
\begin{itemize}[topsep=0pt]
	\setlength\itemsep{-0.1em}
	\item We specify the optimal estimation error under both interactive and non-interactive settings. This is the first result showing the dimension-free convergence rate $O\lp \frac{s}{n2^b}\rp$, and hence closes the gap of upper and lower bounds in \citep{acharya2020estimating}.
	
	\item By proposing novel localization schemes, we give upper bounds on the minimum sample size, which depends only logrithmically on $d$, to achieve the optimal rate.
	
	\item For non-interactive setting, we connect the problem to non-adaptive group testing and obtain a polynomial time decoding algorithm. The proposed scheme is also \emph{adaptive}\footnote{The estimation scheme is said \emph{adaptive} to $s$ if its' design does not require the knowledge of $s$.} to the sparsity parameter $s$.
	
	\item We extend our schemes to several practical scenarios, including estimating almost-sparse distributions and estimating empirical frequencies (i.e. the distribution-free setting).
\end{itemize}

\iffalse
\paragraph{Notation}
We will use the following mathematical notation through the rest of the paper.
\begin{itemize}
	\item We will use $n$ as the number of clients and $d$ as the size of the alphabet $\lba \mcal{X}\rba$.
	\item $[d] \eqDef \lbp 1,...,d \rbp$.
	\item $X^n \eqDef \lp X_1,...,X_n\rp$.
\end{itemize}
\fi

\subsection{Notation and Setup}
%Let $\mcal{P}_d \eqDef \lbp p = (p_1,...,p_d) \, \mv \,  p \in [0, 1]^d, \sum_j p_j =1 \rbp$ be the $d$-dimensional probability simplex, and  $\mcal{P}_{s, d} = \lbp p \in \mcal{P}_d \, \mv \, \lV p \rV_0 \leq s \rbp$ be the collection of all $s$-sparse distributions over $\mcal{P}_d$. For a given $p \in \mcal{P}_{s, d}$, denote the indices of nonzero entries of $p$ by $\mcal{J} = \lbp j_1, j_2,...,j_s\rbp \subset \lbp 1,2,...,d \rbp \eqDef [d]$. 

The general distributed statistical tasks we consider in this paper can be formulated as follows: each one of the $n$ clients has local data $X_i \sim p$ and sends a message $Y_i \in \mcal{Y}$ to the server, who upon receiving $Y^n$ aims to estimate the underlying distribution $p \in \mcal{P}_{s, d}$, where
$$ \mcal{P}_{s, d} \eqDef \lbp p = (p_1,...,p_d) \, \mv \,  p \in [0, 1]^d, \sum_j p_j =1, \lV p \rV_0 \leq s \rbp$$
is the collection of all $d$-dimensional $s$-sparse discrete distributions.

At client $i$, the message $Y_i$ is generated via some encoding channel (a randomized mapping that possibly uses shared randomness across participating clients and the server) denoted by a conditional probability $W_i(\cdot| X_i)$ (for non-interactive setting) or $W_i(\cdot | X_i, Y^{i-1})$ (for interactive setting).  The $b$-bit communication constraint restricts $\lba\mcal{Y}\rba \leq 2^b$, so without loss of generality we assume $\mcal{Y} = [2^b]$. When the context is clear, we sometimes view $W_i$ as a $2^b \times d$ stochastic matrix, with $\lb W_i \rb_{y, x} \eqDef W_i(y|x)$. Finally, we call the tuple $\lp W^n, \hat{p}(Y^n)\rp$ an estimation scheme, where $\hat{p}\lp Y^n \rp$ is an estimator of $p$. 

Let $\Pi_{\msf{smp}}$ be the collection of all non-interactive estimation schemes (i.e. $W_i$ is non-interactive for all $i \in [n]$) and $\Pi_{\msf{seq}}$ be the collection of sequentially interactive schemes. Our goal is to design a scheme $\lp W^n, \hat{p}\lp Y^n \rp\rp$ to minimize the $\ell_2$ (or $\ell_1$) estimation error:
\begin{align*}
	& r_{\msf{smp}}\lp \ell_2, n, b\rp \eqDef \min_{\lp W^n, \hat{p}\rp \in \Pi_{\msf{smp}}} \, \max_{p \in \mcal{P}_{s,d}} \E\lb \left\lVert p - \hat{p}\lp Y^n \rp \right\rVert^2_2 \rb,% \text{ and} \\
	%& r_{\msf{seq}}\lp \ell_2, n, b\rp \eqDef \min_{\lp W^n, \hat{p}\rp \in \Pi_{\msf{seq}}} \, \max_{p \in \mcal{P}_{s,d}} \E\lb \left\lVert p - \hat{p}\lp Y^n \rp \right\rVert^2_2 \rb.
\end{align*}
and $ r_{\msf{seq}}$ defined similarly with the minimum taken in $\Pi_{\msf{seq}}$. For $\ell_1$ error, we replace $\lV \cdot \rV^2_2$ in the above expectations with $\lV \cdot \rV_1$.

%\subsection{Previous results and our contributions}\label{sec:contributions}

\subsection{Related works}\label{sec:related_works}
Estimating discrete distributions is a fundamental task in statistical inference and has a rich literature \citep{barlow1972statistical,devroye1985nonparametric,devroye2012combinatorial,Silverman86}. For estimating discrete distribution under communication constraint, the optimal convergence rate is established in  \citep{han2018geometric, han2018distributed, barnes2019lower, acharya2019inference,  acharya2019inference2, chen2020breaking} for non-interactive setting, and \citep{barnes2019lower, acharya2020general} for general interactive model. 
The recent work \citep{acharya2020estimating} consider the same task under $s$ sparse assumption with communication or privacy constraints. However, their result for communication constraint has a $\log\lp\frac{d}{s}\rp$ gap between the upper and the lower bounds.

A slightly different but closely related problem is distributed heavy hitter detection under LDP constraints \citep{Bassily2015, Bassily2017, bun2019heavy, zhu2020federated} where no distributional assumption on the data is made. Although originally designed for preserving user privacy, the non-interactive tree-based schemes proposed in \citep{Bassily2017, bun2019heavy} can be modified to communication efficient (indeed $1$-bit) distribution estimation schemes. However, in the heavy-hitter problem, most of the results optimize with respect to $\ell_\infty$ error, and directly applying their frequency oracles leads to a sub-optimal convergence $O\lp \frac{s(\log d+ \log n)}{n}\rp$ in $\ell_2$ (see Section~\ref{sec:decoding} for a brief discussion). On the other hand, the interactive scheme in \citep{zhu2020federated}, which identifies (instead of estimating the frequencies of) heavy-hitter symbols, is similar to our proposed interactive scheme in nature. Nevertheless, we extend their result to a communication efficient scheme and explicitly characterize the convergence rate.

In our construction of a non-interactive polynomial-time decodable scheme (Section~\ref{sec:ncgt}), we map the support localization task into the non-adaptive combinatorial group testing problem \citep{dorfman1943detection, du2000combinatorial, ngo2000survey}. In particular, we show that the Kautz and Singleton's construction of test measurement matrices \citep{kautz1964nonrandom} can be used to design the local encoding channels and obtain a polynomial time decoding algorithm at the cost of a slightly larger sample size requirement.


